Red Bots Do It Better: Comparative Analysis of Social Bot Partisan Behavior

Recent research brought awareness of the issue of bots on social media and the significant risks of mass manipulation of public opinion in the context of political discussion. In this work, we leverage Twitter to study the discourse during the 2018 US midterm elections and analyze social bot activity and interactions with humans. We collected 2.6 million tweets for 42 days around the election day from nearly 1 million users. We use the collected tweets to answer three research questions: (i) Do social bots lean and behave according to a political ideology? (ii) Can we observe different strategies among liberal and conservative bots? (iii) How effective are bot strategies? We show that social bots can be accurately classified according to their political leaning and behave accordingly. Conservative bots share most of the topics of discussion with their human counterparts, while liberal bots show less overlap and a more inflammatory attitude. We studied bot interactions with humans and observed different strategies. Finally, we measured bots embeddedness in the social network and the effectiveness of their activities. Results show that conservative bots are more deeply embedded in the social network and more effective than liberal bots at exerting influence on humans.

==> src/notepad.tex <==
Likewise, there are a number of ways to infer the political ideology of a social media account. Given how divided much of the media oultets are, we can classify users based the the political leaning of the media organization. 


We use lists of partisan media outlets compiled by third-party organizations, such as AllSides\footnote{\url{https://www.allsides.com/media-bias/media-bias-ratings}} and Media Bias/Fact Check.\footnote{\url{https://mediabiasfactcheck.com/}}

Anything left of center we classify as liberal and anything right of center we classify as conservative the combined list has 641 liberal and 398 conservative outlets.


We classify users by their ideology based on the political leaning of the media outlets they share. %The classification algorithm is described in Section \textcolor{red}{sec:labelpropagation}. In this section, We describe the methodology of obtaining ground truth labels for the media outlets.

Twitter shortens the full URL for links in tweets and we require the extended URL for our analysis. Since the reverse of this process can be time intensive, we select the 5,000 most popular short URLs and then recover the long version from them. The 5,000 URLs represent one-third of all the URLs given that there were ~250K shortened, unique URLs in the dataset. 


After cross-referencing the 5,000 long URLs with the media outlets, we observe that 32,115 tweets in the dataset contain a URL that refers to one of the liberal media outlets and 25,273 tweets with a URL referring to one of the conservative media outlets. 
% Figure \ref{fig:media}  shows the distributions of tweets with URLs from liberal and conservative outlets. As we can see in the figures, thegatewaypundit.com and breitbart.com are the most shared  URLs in the conservative sample, while in the liberal sample the hill.com dominated. 
% 
% 
% \begin{figure*}
%   \includegraphics[width=0.5\textwidth]{LaTeX/src/left_media_dist.png}
%   \includegraphics[width=0.5\textwidth]{LaTeX/src/right_media_dist.png}
% \caption{Distribution of tweets with links to liberal (right) and conservative (left) media outlets.}
% \label{fig:media}   
% \end{figure*}
% 


If a user has more tweets with a URL linking to liberal sources, that account is labeled as liberal; likewise, if a user has more tweets linking to conservative, that user is labeled as conservative. 


In essence, use a polarity rule to label Twitter users as liberal or conservative. 

Although the vast majority of users include URLs that are either liberal or conservative, we remove any ties, such that a user has equal number of tweets from each side. Our final set of labeled users includes 38,920 users.

% \begin{table}[tbp]
% \centering
% \caption{Descriptive statistics of the Retweet Network.}
% \label{Tab:RetweetNetwork}
% \begin{tabular}{|l|c|c|c|}
% \hline
% Statstic       & Count      \\ 
% \hline
% \# of nodes    &  771,905 \\
% \# of edges    & 1,754,634 \\
% Max in-degree  &  39,017 \\
% Max out-degree &  215\\
% Density        & 2.9e-06 \\ 
% \hline
% \end{tabular}
% \end{table}


We classify the remaining accounts as liberal or conservative using label propagation, similar to prior work in \cite{Badawy2018}. 

Label propagation is a network science method so we construct a retweet network, where each node is a Twitter user and the edges are directed from the user who retweets (source) to the user who was retweeted (destination). This network has as many nodes as users (authors plus mentions) and as many links as retweets.   %Table \ref{Tab:RetweetNetwork} shows the descriptive statistics of the retweet network. It is a sparse network with a giant component that includes 708,363 nodes.
To validate results of the label propagation, we apply stratified cross (5-fold) validation to a set of more than 38,920 seeds. We train the algorithm on 80\% of the seed list and see how it performs on the remaining 20\% of the seed list. 

Both precision and recall scores are approximately 89\%. 
The algorithm performs well despite the earlier merging of liberal and liberal-center as well as the conservative and conservative-center. 

%Since we combine liberal and liberal-center into one list (same for conservatives), we can see that the algorithm is not only labeling the far liberal or conservative correctly, which is a relatively easier task, but it is performing well on the liberal/conservative center as well. 

==> src/related_work.tex <==
%%%%%%%% call for papers %%%%%%%%%%%%%
%Our society is struggling with an unprecedented amount of falsehood which harms wealth, democracy, and health.
% The last  few years have witnessed a substantial growth in efforts at computational fact-checking, of which many are data-driven, AI-powered, and include human in the loop. 
These efforts tackle various fronts, such as the detection of fabricated news, rumors, and spam on social media, automation in fact-checking, flagging clickbait articles, and discovering fake accounts and malicious social media bots. 

 we must raise the awareness of all aspects about misinformation and we must train a generation of Web users that are well versed in media literacy, data literacy, and logic and fallacy. 
 
 solutions to mitigate the challenges posed by malicious adversaries who misuse advanced computing and AI technologies
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

During the last decade, social media have become the conventional communication medium to connect with people, share opinions, and, particularly in the last few years, to find news.
For this reason, the truthfulness and the authenticity of the shared content are the necessary ingredients to maintain a healthy online discussion.
However, in the last few years, social media are dealing with a considerable growth of false content and fake accounts.
The resulting wave of misinformation (and disinformation) highlights the pitfalls of social media networks like Twitter and Facebook on the one hand, while on the other hand harms several constituent of our society ranging from politics to health.

In fact, social media networks have been used for malicious purposes to a great extent \cite{ferrara2015manipulation}. %Especially in the context of political discussion, there is a significant risk of mass manipulation of public opinion.
Numerous studies raised awareness about the risk of mass manipulation of public opinion, especially in the context of political discussion.
Disinformation~\cite{persily20172016, howard2017junk, shu2017fake, vosoughi2018spread, badawy2018falls, guess2019less, bovet2019influence, scheufele2019science, Grinberg2019}, social media bots~\cite{bessi2016social, woolley2017computational, varol2017online, monsted2017evidence, boichak2018automated, shao2018spread, yang2019arming}, and polarization \cite{bail2018exposure, azzimonti2018social} are just few factors that drive political manipulation in social media.
% Especially for the spread of fake news, various studies showed how political leaning \cite{allcott2017social}, age \cite{Grinberg2019}, and education \cite{scheufele2019science} can greatly affect fake news spread, alongside with other mechanisms that leverage emotions \cite{ferrara2015quantifying, ferrara2015measuring} and cognitive limits \cite{PENNYCOOK2018, pennycook2019cognitive}. 
% Additionally, \citet{dutt2018senator} showed how foreign actors can more so than just backing one candidate or the other often manipulate social media for the purpose of sowing discord. 

In particular, the 2016 US Presidential election represent the prime example of the significant perils of mass manipulation in the political discourse. 
\citet{Badawy2018} studied the Russian interference in the election and the activity of Russian trolls on Twitter. As \citet{im2019still} showed, troll accounts are believed to be still active to these days.
On the same wavelength, the presence of social bots does not show signs of decline \citet{yang2019arming,deb2019bots} despite the attempt from social network companies to suspend the suspected (malicious) accounts.
Complementary, research efforts are focused on the analysis, detection, and countermeasures development against social bots.
\citet{ferrara2016rise} brought awareness to the issue of social bots in social media platforms, while in \cite{bessi2016social}, Bessi \& Ferrara focused on social bots detection within the online discussion related to the 2016 presidential election.



\citet{shao2018spread} bots have a remarkable role in spreading articles from low credability sources.
More recently, \citet{stella2018bots} highlighted how bots can play significant roles in targeting influential humans to manipulate online discussion thus increasing in-fighting. Recently, Deb et al. \cite{deb2019bots} focused on the 2018 Midterms election by using a large collection of data sources. In their work, they seek to find voter issues and anomalies, whereas here we investigate social bots, analyzing their strategies and interactions with humans. 







%In this paper, we address the potential malicious activity in online political discussion along the lines of voter fraud, voter suppression, political misinformation, and then report on the biases we found. 
%In this work, we leverageTwitter to study the discourse during the 2018 US midterm electionsand analyze social bot activity and interactions with humans. Wecollected 2.6 million tweets for 42 days around the election day fromnearly 1 million users. We use the collected tweets to answer thr
% \subsection{Research Questions}
In this paper, we aim to answer the following research questions (RQs) regarding social bots behavior during the 2018 Midterms election. 
